Advantage Matching: A General Reinforcement Learning Framework for LLM Reasoning

Reinforcement learning (RL) has emerged as a promising paradigm for improving reasoning in large language models (LLMs), enabling models to optimize full reasoning trajectories using task-level feedback. However, existing RL-based approaches suffer from several limitations, including reliance on surrogate objectives and approximate advantage estimators, token-level optimization that overlooks trajectory-level dependencies, and predominantly on-policy training that restricts the utilization of offline data. We introduce \textbf{Advantage Matching}, a general framework for KL-regularized RL that leverages the principled relationship between the policy ratio and the soft advantage to learn the optimal policy by aligning the two quantities. Our formulation yields a family of stable and flexible objectives that support critic-free optimization, trajectory-level reasoning, and seamless integration of off-policy and offline data. Empirical results on diverse mathematical reasoning and code generation benchmarks and model families show improvements in performance of our method compared to existing baselines.

==> checklist.tex <==

\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible
machine learning research, addressing issues of reproducibility, transparency,
research ethics, and societal impact. Do not remove the checklist:
\textbf{The papers not including the checklist will be desk rejected.}
The checklist should follow the references and follow the (optional)
supplemental material. The checklist does NOT count towards the page
limit.

Please read the checklist guidelines carefully for information on
how to answer these questions. For each question in the checklist: 
\begin{itemize}
\item You should answer \answerYes{}, \answerNo{}, or \answerNA{}. 
\item \answerNA{} means either that the question is Not Applicable for
that particular paper or the relevant information is Not Available. 
\item Please provide a short (1--2 sentence) justification right after
your answer (even for \answerNA). % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}
\textbf{The checklist answers are an integral part of your paper submission.}
They are visible to the reviewers, area chairs, senior area chairs,
and ethics reviewers. You will also be asked to include it (after
eventual revisions) with the final version of your paper, and its
final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as
one of the factors in their evaluation. While \answerYes{} is generally
preferable to \answerNo{}, it is perfectly acceptable to answer
\answerNo{} provided a proper justification is given (e.g., error
bars are not reported because it would be too computationally expensive''
or ``we were unable to find the license for the dataset we used'').
In general, answering \answerNo{} or \answerNA{} is not grounds
for rejection. While the questions are phrased in a binary way, we
acknowledge that the true answer is often more nuanced, so please
just use your best judgment and write a justification to elaborate.
All supporting evidence can appear either in the main paper or the
supplemental material, provided in appendix. If you answer \answerYes{}
to a question, in the justification please point to the section(s)
where related material for the question can be found.

IMPORTANT, please: 
\begin{itemize}
\item \textbf{Delete this instruction block, but keep the section heading
``NeurIPS Paper Checklist"}, 
\item \textbf{Keep the checklist subsection headings, questions/answers
and guidelines below.} 
\item \textbf{Do not modify the questions and only use the provided macros
for your answers}. 
\end{itemize}
%%% END INSTRUCTIONS %%%
\begin{enumerate}
\par 
\item \textbf{Claims} 
\item[] Question: Do the main claims made in the abstract and introduction
accurately reflect the paper's contributions and scope? 
\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: The main claims in the abstract and introduction accurately
reflect the paper's contributions and scope.
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the abstract and introduction
do not include the claims made in the paper. 
\item The abstract and/or introduction should clearly state the claims made,
including the contributions made in the paper and important assumptions
and limitations. A \answerNo{} or \answerNA{} answer to this question
will not be perceived well by the reviewers. 
\item The claims made should match theoretical and experimental results,
and reflect how much the results can be expected to generalize to
other settings. 
\item It is fine to include aspirational goals as motivation as long as
it is clear that these goals are not attained by the paper. 
\end{itemize}
\item \textbf{Limitations} 
\item[] Question: Does the paper discuss the limitations of the work performed
by the authors? 
\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: The limitation is clearly discussed in the Conclusion
section
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper has no limitation while
the answer \answerNo{} means that the paper has limitations, but
those are not discussed in the paper. 
\item The authors are encouraged to create a separate ``Limitations''
section in their paper. 
\item The paper should point out any strong assumptions and how robust the
results are to violations of these assumptions (e.g., independence
assumptions, noiseless settings, model well-specification, asymptotic
approximations only holding locally). The authors should reflect on
how these assumptions might be violated in practice and what the implications
would be. 
\item The authors should reflect on the scope of the claims made, e.g.,
if the approach was only tested on a few datasets or with a few runs.
In general, empirical results often depend on implicit assumptions,
which should be articulated. 
\item The authors should reflect on the factors that influence the performance
of the approach. For example, a facial recognition algorithm may perform
poorly when image resolution is low or images are taken in low lighting.
Or a speech-to-text system might not be used reliably to provide closed
captions for online lectures because it fails to handle technical
jargon. 
\item The authors should discuss the computational efficiency of the proposed
algorithms and how they scale with dataset size. 
\item If applicable, the authors should discuss possible limitations of
their approach to address problems of privacy and fairness. 
\item While the authors might fear that complete honesty about limitations
might be used by reviewers as grounds for rejection, a worse outcome
might be that reviewers discover limitations that aren't acknowledged
in the paper. The authors should use their best judgment and recognize
that individual actions in favor of transparency play an important
role in developing norms that preserve the integrity of the community.
Reviewers will be specifically instructed to not penalize honesty
concerning limitations. 
\end{itemize}
\item \textbf{Theory assumptions and proofs} 
\item[] Question: For each theoretical result, does the paper provide the
full set of assumptions and a complete (and correct) proof? 
\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: All proofs are clearly presented in the Appendix
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper does not include theoretical
results. 
\item All the theorems, formulas, and proofs in the paper should be numbered
and cross-referenced. 
\item All assumptions should be clearly stated or referenced in the statement
of any theorems. 
\item The proofs can either appear in the main paper or the supplemental
material, but if they appear in the supplemental material, the authors
are encouraged to provide a short proof sketch to provide intuition. 
\item Inversely, any informal proof provided in the core of the paper should
be complemented by formal proofs provided in appendix or supplemental
material. 
\item Theorems and Lemmas that the proof relies upon should be properly
referenced. 
\end{itemize}
\item \textbf{Experimental result reproducibility} 
\item[] Question: Does the paper fully disclose all the information needed
to reproduce the main experimental results of the paper to the extent
that it affects the main claims and/or conclusions of the paper (regardless
of whether the code and data are provided or not)? 
\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: Yes, please check the Experimental Setup section and
our discussion of experimental results
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper does not include experiments. 
\item If the paper includes experiments, a \answerNo{} answer to this
question will not be perceived well by the reviewers: Making the paper
reproducible is important, regardless of whether the code and data
are provided or not. 
\item If the contribution is a dataset and\slash or model, the authors should
describe the steps taken to make their results reproducible or verifiable. 
\item Depending on the contribution, reproducibility can be accomplished
in various ways. For example, if the contribution is a novel architecture,
describing the architecture fully might suffice, or if the contribution
is a specific model and empirical evaluation, it may be necessary
to either make it possible for others to replicate the model with
the same dataset, or provide access to the model. In general. releasing
code and data is often one good way to accomplish this, but reproducibility
can also be provided via detailed instructions for how to replicate
the results, access to a hosted model (e.g., in the case of a large
language model), releasing of a model checkpoint, or other means that
are appropriate to the research performed. 
\item While NeurIPS does not require releasing code, the conference does
require all submissions to provide some reasonable avenue for reproducibility,
which may depend on the nature of the contribution. For example 
\begin{enumerate}
\item If the contribution is primarily a new algorithm, the paper should
make it clear how to reproduce that algorithm. 
\item If the contribution is primarily a new model architecture, the paper
should describe the architecture clearly and fully. 
\item If the contribution is a new model (e.g., a large language model),
then there should either be a way to access this model for reproducing
the results or a way to reproduce the model (e.g., with an open-source
dataset or instructions for how to construct the dataset). 
\item We recognize that reproducibility may be tricky in some cases, in
which case authors are welcome to describe the particular way they
provide for reproducibility. In the case of closed-source models,
it may be that access to the model is limited in some way (e.g., to
registered users), but it should be possible for other researchers
to have some path to reproducing or verifying the results. 
\end{enumerate}
\end{itemize}
\item \textbf{Open access to data and code} 
\item[] Question: Does the paper provide open access to the data and code,
with sufficient instructions to faithfully reproduce the main experimental
results, as described in supplemental material? 
\item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: We haven't had enough time to prepare source code
and will provide later. However, detail configurations were provided
to ensure results are reproducible
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that paper does not include experiments
requiring code. 
\item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy})
for more details. 
\item While we encourage the release of code and data, we understand that
this might not be possible, so \answerNo{} is an acceptable answer.
Papers cannot be rejected simply for not including code, unless this
is central to the contribution (e.g., for a new open-source benchmark). 
\item The instructions should contain the exact command and environment
needed to run to reproduce the results. See the NeurIPS code and data
submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy})
for more details. 
\item The authors should provide instructions on data access and preparation,
including how to access the raw data, preprocessed data, intermediate
data, and generated data, etc. 
\item The authors should provide scripts to reproduce all experimental results
for the new proposed method and baselines. If only a subset of experiments
are reproducible, they should state which ones are omitted from the
script and why. 
\item At submission time, to preserve anonymity, the authors should release
anonymized versions (if applicable). 
\item Providing as much information as possible in supplemental material
(appended to the paper) is recommended, but including URLs to data
and code is permitted. 
\end{itemize}
\item \textbf{Experimental setting/details} 
\item[] Question: Does the paper specify all the training and test details
(e.g., data splits, hyperparameters, how they were chosen, type of
optimizer) necessary to understand the results? 
\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: Please check our Experimental Setup section
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper does not include experiments. 
\item The experimental setting should be presented in the core of the paper
to a level of detail that is necessary to appreciate the results and
make sense of them. 
\item The full details can be provided either with the code, in appendix,
or as supplemental material. 
\end{itemize}
\item \textbf{Experiment statistical significance} 
\item[] Question: Does the paper report error bars suitably and correctly
defined or other appropriate information about the statistical significance
of the experiments? 
\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: Because RL training exhibits substantial fluctuations
throughout optimization, computing standard deviations from the final
checkpoints of multiple runs may not accurately reflect training behavior.
Instead of reporting error bars, we track evaluation performance across
training iterations and visualize the resulting curves, which more
clearly illustrate the learning dynamics of our method relative to
the baselines.
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper does not include experiments. 
\item The authors should answer \answerYes{} if the results are accompanied
by error bars, confidence intervals, or statistical significance tests,
at least for the experiments that support the main claims of the paper. 
\item The factors of variability that the error bars are capturing should
be clearly stated (for example, train/test split, initialization,
random drawing of some parameter, or overall run with given experimental
conditions). 
\item The method for calculating the error bars should be explained (closed
form formula, call to a library function, bootstrap, etc.) 
\item The assumptions made should be given (e.g., Normally distributed errors). 
\item It should be clear whether the error bar is the standard deviation
or the standard error of the mean. 
\item It is OK to report 1-sigma error bars, but one should state it. The
authors should preferably report a 2-sigma error bar than state that
they have a 96\% CI, if the hypothesis of Normality of errors is not
verified. 
\item For asymmetric distributions, the authors should be careful not to
show in tables or figures symmetric error bars that would yield results
that are out of range (e.g., negative error rates). 
\item If error bars are reported in tables or plots, the authors should
explain in the text how they were calculated and reference the corresponding
figures or tables in the text. 
\end{itemize}
\item \textbf{Experiments compute resources} 
\item[] Question: For each experiment, does the paper provide sufficient
information on the computer resources (type of compute workers, memory,
time of execution) needed to reproduce the experiments? 
\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: Please see the Experimental Setup section
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper does not include experiments. 
\item The paper should indicate the type of compute workers CPU or GPU,
internal cluster, or cloud provider, including relevant memory and
storage. 
\item The paper should provide the amount of compute required for each of
the individual experimental runs as well as estimate the total compute. 
\item The paper should disclose whether the full research project required
more compute than the experiments reported in the paper (e.g., preliminary
or failed experiments that didn't make it into the paper). 
\end{itemize}
\item \textbf{Code of ethics} 
\item[] Question: Does the research conducted in the paper conform, in every
respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}? 
\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: All authors adhere to the NeurIPS Code of Ethics,
and the research presented in this work was conducted in accordance
with its principles.
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the authors have not reviewed
the NeurIPS Code of Ethics. 
\item If the authors answer \answerNo, they should explain the special
circumstances that require a deviation from the Code of Ethics. 
\item The authors should make sure to preserve anonymity (e.g., if there
is a special consideration due to laws or regulations in their jurisdiction). 
\end{itemize}
\item \textbf{Broader impacts} 
\item[] Question: Does the paper discuss both potential positive societal
impacts and negative societal impacts of the work performed? 
\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: There is not negative societal impact with the current
work.
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that there is no societal impact of
the work performed. 
\item If the authors answer \answerNA{} or \answerNo, they should explain
why their work has no societal impact or why the paper does not address
societal impact. 
\item Examples of negative societal impacts include potential malicious
or unintended uses (e.g., disinformation, generating fake profiles,
surveillance), fairness considerations (e.g., deployment of technologies
that could make decisions that unfairly impact specific groups), privacy
considerations, and security considerations. 
\item The conference expects that many papers will be foundational research
and not tied to particular applications, let alone deployments. However,
if there is a direct path to any negative applications, the authors
should point it out. For example, it is legitimate to point out that
an improvement in the quality of generative models could be used to
generate Deepfakes for disinformation. On the other hand, it is not
needed to point out that a generic algorithm for optimizing neural
networks could enable people to train models that generate Deepfakes
faster. 
\item The authors should consider possible harms that could arise when the
technology is being used as intended and functioning correctly, harms
that could arise when the technology is being used as intended but
gives incorrect results, and harms following from (intentional or
unintentional) misuse of the technology. 
\item If there are negative societal impacts, the authors could also discuss
possible mitigation strategies (e.g., gated release of models, providing
defenses in addition to attacks, mechanisms for monitoring misuse,
mechanisms to monitor how a system learns from feedback over time,
improving the efficiency and accessibility of ML). 
\end{itemize}
\item \textbf{Safeguards} 
\item[] Question: Does the paper describe safeguards that have been put in
place for responsible release of data or models that have a high risk
for misuse (e.g., pre-trained language models, image generators, or
scraped datasets)? 
\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: The paper poses no such risks. 
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper poses no such risks. 
\item Released models that have a high risk for misuse or dual-use should
be released with necessary safeguards to allow for controlled use
of the model, for example by requiring that users adhere to usage
guidelines or restrictions to access the model or implementing safety
filters. 
\item Datasets that have been scraped from the Internet could pose safety
risks. The authors should describe how they avoided releasing unsafe
images. 
\item We recognize that providing effective safeguards is challenging, and
many papers do not require this, but we encourage authors to take
this into account and make a best faith effort. 
\end{itemize}
\item \textbf{Licenses for existing assets} 
\item[] Question: Are the creators or original owners of assets (e.g., code,
data, models), used in the paper, properly credited and are the license
and terms of use explicitly mentioned and properly respected? 
\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: Please refer to our Experimental Setup section
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper does not use existing
assets. 
\item The authors should cite the original paper that produced the code
package or dataset. 
\item The authors should state which version of the asset is used and, if
possible, include a URL. 
\item The name of the license (e.g., CC-BY 4.0) should be included for each
asset. 
\item For scraped data from a particular source (e.g., website), the copyright
and terms of service of that source should be provided. 
\item If assets are released, the license, copyright information, and terms
of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets}
has curated licenses for some datasets. Their licensing guide can
help determine the license of a dataset. 
\item For existing datasets that are re-packaged, both the original license
and the license of the derived asset (if it has changed) should be
provided. 
\item If this information is not available online, the authors are encouraged
to reach out to the asset's creators. 
\end{itemize}
\item \textbf{New assets} 
\item[] Question: Are new assets introduced in the paper well documented
and is the documentation provided alongside the assets? 
\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: The paper does not release new assets. 
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper does not release new
assets. 
\item Researchers should communicate the details of the dataset\slash code\slash model
as part of their submissions via structured templates. This includes
details about training, license, limitations, etc. 
\item The paper should discuss whether and how consent was obtained from
people whose asset is used. 
\item At submission time, remember to anonymize your assets (if applicable).
You can either create an anonymized URL or include an anonymized zip
file. 
\end{itemize}
\item \textbf{Crowdsourcing and research with human subjects} 
\item[] Question: For crowdsourcing experiments and research with human subjects,
does the paper include the full text of instructions given to participants
and screenshots, if applicable, as well as details about compensation
(if any)? 
\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: The paper does not involve crowdsourcing nor research
with human subjects. 
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper does not involve crowdsourcing
nor research with human subjects. 
\item Including this information in the supplemental material is fine, but
if the main contribution of the paper involves human subjects, then
as much detail as possible should be included in the main paper. 
\item According to the NeurIPS Code of Ethics, workers involved in data
collection, curation, or other labor should be paid at least the minimum
wage in the country of the data collector. 
\end{itemize}
\item \textbf{Institutional review board (IRB) approvals or equivalent for
research with human subjects} 
\item[] Question: Does the paper describe potential risks incurred by study
participants, whether such risks were disclosed to the subjects, and
whether Institutional Review Board (IRB) approvals (or an equivalent
approval/review based on the requirements of your country or institution)
were obtained? 
\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: The paper does not involve crowdsourcing nor research
with human subjects. 
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the paper does not involve crowdsourcing
nor research with human subjects. 
\item Depending on the country in which research is conducted, IRB approval
(or equivalent) may be required for any human subjects research. If
you obtained IRB approval, you should clearly state this in the paper. 
\item We recognize that the procedures for this may vary significantly between
institutions and locations, and we expect authors to adhere to the
NeurIPS Code of Ethics and the guidelines for their institution. 
\item For initial submissions, do not include any information that would
break anonymity (if applicable), such as the institution conducting
the review. 
\end{itemize}
\item \textbf{Declaration of LLM usage} 
\item[] Question: Does the paper describe the usage of LLMs if it is an important,
original, or non-standard component of the core methods in this research?
Note that if the LLM is used only for writing, editing, or formatting
purposes and does \emph{not} impact the core methodology, scientific
rigor, or originality of the research, declaration is not required.
%this research? 
 
\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
 
\item[] Justification: The core method development in this research does
not involve LLMs as any important, original, or non-standard components. 
\item[] Guidelines: 
\begin{itemize}
\item The answer \answerNA{} means that the core method development in
this research does not involve LLMs as any important, original, or
non-standard components. 
\item Please refer to our LLM policy in the NeurIPS handbook for what should
or should not be described. 
\end{itemize}
\end{enumerate}


